Rational cohomology of $\mathcal M_{4,1}$

We compute the rational cohomology of the moduli space $\mathcal{M}_{4,1}$ of non-singular genus $4$ curves with $1$ marked point, using Gorinov-Vassiliev's method.

==> pre.tex <==
\RequirePackage{filecontents}




\usepackage{tabto}
\usepackage{imakeidx}
\usepackage[normalem]{ulem}
\usepackage{cleveref}

\numberwithin{equation}{section}

%% Theorem environments
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lm}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{add}[thm]{Addendum}
\newtheorem{fact}[thm]{Fact}
\newtheorem{qu}[thm]{Question}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{summary}[thm]{Summary}
\theoremstyle{definition}
\newtheorem{dfx}[thm]{Definition}
\newtheorem{alg}[thm]{Algorithm}
\newtheorem{assu}[thm]{Assumption}
\newenvironment{df}
{\pushQED{\qed}\renewcommand{\qedsymbol}{$\triangle$}\dfx}
{\popQED\enddfx}

%\renewcommand{\qedsymbol}{\manimpossiblecube}


\newtheorem{notat}[thm]{Notation}
\newtheorem{rem}[thm]{Remark}
\newtheorem{exa}[thm]{Example}

\newtheorem{ass}{Assumption}


%%%%%%%%%%%%%% equations
\def\={\;=\;}  \def\+{\,+\,} \def\m{\,-\,}
\def\ve{\epsilon}
\def\vare{\varepsilon}
\def\be{\begin{equation}}   \def\ee{\end{equation}}     \def\bes{\begin{equation*}}    \def\ees{\end{equation*}}
\def\ba{\be\begin{aligned}} \def\ea{\end{aligned}\ee}   \def\bas{\bes\begin{aligned}}  \def\eas{\end{aligned}\ees}

\DeclareRobustCommand{\rchi}{{\mathpalette\irchi\relax}}
\newcommand{\irchi}[2]{\raisebox{\depth}{$#1\chi$}} % inner command, used by \rchi
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Lan}{Lan}
\DeclareMathOperator{\Ran}{Ran}
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\ord}{ord}
\DeclareMathOperator{\unord}{unord}
\DeclareMathOperator{\ordin}{ordin}
\DeclareMathOperator{\hflx}{hflx}
\DeclareMathOperator{\flx}{flx}
\DeclareMathOperator{\BM}{BM}
\DeclareMathOperator{\hyp}{hyp}
\DeclareMathOperator{\non}{non}
\DeclareMathOperator{\Conf}{Conf}
\DeclareMathOperator{\Sing}{Sing}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\Gr}{Gr}
\DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\Jac}{Jac}
\DeclareMathOperator{\res}{res}
\DeclareMathOperator{\ind}{ind}
\DeclareMathOperator{\divisor}{div}
\DeclareMathOperator{\Image}{Im}
\DeclareMathOperator{\Bl}{Bl}
\DeclareMathOperator{\pr}{pr}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\btg}{btg}
\DeclareMathOperator{\DR}{DR}
\DeclareMathOperator{\LG}{LG}
\DeclareMathOperator{\PGL}{PGL}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\rank}{rank}
\newcommand*\oline[1]{%
  \vbox{%
    \hrule height 0.5pt%                  % Line above with certain width
    \kern0.25ex%                          % Distance between line and content
    \hbox{%
      \kern-0.15em%                        % Distance between content and left side of box, negative values for lines shorter than content
      \ifmmode#1\else\ensuremath{#1}\fi%  % The content, typeset in dependence of mode
      \kern-0.05em%                        % Distance between content and left side of box, negative values for lines shorter than content
    }% end of hbox
  }% end of vbox
}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\PP}{\mathbb{P}}


\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\barmoduli}{\overline{\cM}_{g,n}}
\newcommand{\moduli}{\cM_{g,n}}
\newcommand{\omoduli}{\Omega\cM_{g,n}(\mu)}
\newcommand{\pomoduli}{\PP\Omega\cM_{g,n}(\mu)}
\newcommand{\poxmoduli}{\PP\Xi\overline{\cM}_{g,n}(\mu)}
\newcommand{\momoduli}{\Omega\cM_{\boldsymbol{g},\boldsymbol{n}}(\boldsymbol{\mu})}
\newcommand{\pmomoduli}{\PP\Omega\cM_{\boldsymbol{g},\boldsymbol{n}}(\boldsymbol{\mu})}
\newcommand{\pmoxmoduli}{\PP\Xi\overline{\cM}_{\boldsymbol{g},\boldsymbol{n}}(\boldsymbol{\mu})}
\newcommand{\pmoxrmoduli}{\PP\Xi\overline{\cM} ^\mathfrak{R}_{\boldsymbol{g},\boldsymbol{n}}(\boldsymbol{\mu})}

\DeclareFontFamily{U}{BOONDOX-calo}{\skewchar\font=45 }
\DeclareFontShape{U}{BOONDOX-calo}{m}{n}{
  <-> s*[1.05] BOONDOX-r-calo}{}
\DeclareFontShape{U}{BOONDOX-calo}{b}{n}{
  <-> s*[1.05] BOONDOX-b-calo}{}
\DeclareMathAlphabet{\mathcalboondox}{U}{BOONDOX-calo}{m}{n}
\SetMathAlphabet{\mathcalboondox}{bold}{U}{BOONDOX-calo}{b}{n}
\DeclareMathAlphabet{\mathbcalboondox}{U}{BOONDOX-calo}{b}{n}

\newcommand{\An}[1]{{\color{blue} Angelina: #1}}
\newcommand{\Ym}[1]{{\color{red} Yiu Man: #1}}
\newcommand{\Ra}[1]{{\color{green} Raluca: #1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\defbb#1{\expandafter\def\csname b#1\endcsname{\mathbb{#1}}}
\def\defcal#1{\expandafter\def\csname c#1\endcsname{\mathcal{#1}}}
\def\deffrak#1{\expandafter\def\csname frak#1\endcsname{\mathfrak{#1}}}
\def\defop#1{\expandafter\def\csname#1\endcsname{\operatorname{#1}}}
\def\defbf#1{\expandafter\def\csname b#1\endcsname{\mathbf{#1}}}

\makeatletter
\def\defcals#1{\@defcals#1\@nil}
\def\@defcals#1{\ifx#1\@nil\else\defcal{#1}\expandafter\@defcals\fi}
\def\deffraks#1{\@deffraks#1\@nil}
\def\@deffraks#1{\ifx#1\@nil\else\deffrak{#1}\expandafter\@deffraks\fi}
\def\defbbs#1{\@defbbs#1\@nil}
\def\@defbbs#1{\ifx#1\@nil\else\defbb{#1}\expandafter\@defbbs\fi}
\def\defbfs#1{\@defbfs#1\@nil}
\def\@defbfs#1{\ifx#1\@nil\else\defbf{#1}\expandafter\@defbfs\fi}
\def\defops#1{\@defops#1,\@nil}
\def\@defops#1,#2\@nil{\if\relax#1\relax\else\defop{#1}\fi\if\relax#2\relax\else\expandafter\@defops#2\@nil\fi}
\makeatother



%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Benutzerteil: %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\defbbs{ZHQCNPALRVW}
\defcals{ABOPQMNXYLTRAEHZKCFI}
\deffraks{apijklmnopqueRC}
\defops{IVC, PGL,SL,mod,Spec,Re,Gal,Tr,End,GL,Hom,PSL,H,div,Aut,rk,Mod,R,T,Tr,Mat,Vol,MV,Res,vol,Z,diag,Hyp,hyp,hl,ord,Im,ev,U,dev,c,CH,fin,pr,Pic,lcm,ch,td,LG,id,Sym,Aut,Log,tw,PS}
\defbfs{uvzwp} % only use this for small letters, otherwise you go directly to hell!!!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ep{\varepsilon}
\def\ve{\varepsilon}
